Weak MSO+U with Path Quantifiers over Infinite Trees

This paper shows that over infinite trees, satisfiability is decidable for weak monadic second-order logic extended by the unbounding quantifier U and quantification over infinite paths. The proof is by reduction to emptiness for a certain automaton model, while emptiness for the automaton model is decided using profinite trees.

==> rubbish.tex <==
 In this part of the appendix, we define an automaton model that has the same expressive power as existential \wmsoup, which is called a \emph{nested \wmsoup automaton}. 
The automaton model is obtained by nesting two kinds of atomic automata, called \emph{atomic prefix automata} and \emph{atomic counter automata}. 







\subsection{Nested counter automata and transducers.} 
In this section, we show that every \wmsoup formula can be converted into an equivalent \wmsoup automaton. The proof is by induction on the size of the formula; the key step is the quantifiers. Instead of the unbounding quantifier, we will use the   \emph{chain unbounding quantification},  where  $\mathsf U_{\mathrm{chain}} X \varphi(X)$ says that $\varphi(X)$ holds for arbitrarily large chains, i.e.~not necessarily connected subsets of paths.

\begin{lemma}\label{lem:}
	Replacing the unbounding quantifier by the chain unbounding quantifier does not affect the expressive power of \wmsoup.
\end{lemma}
\begin{mproof}
	Being a chain is definable in \wmsoup, even first-order logic, so the chain unbounding quantifier does not increase expressive power. For the converse reduction, we use the notion of a spine. 
We say a chain $Y$ is a \emph{spine} of a set $X$ if for every two elements $x < y$ of $Y$, there is some element of $X$ that is a descendant of $x$ but not of $y$.  Instead of saying that $\varphi(X)$ is true for arbitrarily large sets $X$, we say that there are arbitrarily large sets $Y$, such that $Y$ is a spine of some set satisfying $\varphi(X)$.
\end{mproof}

Following standard practice, to show that automata are closed under quantifiers, we encode free variables into the trees. 
 To encode a set of nodes $X$ in a tree $t$ over alphabet $A$, we write $t \otimes X$ for the tree over alphabet $A \times \set{0,1}$ obtained from $t$ by extending the label of every node by a bit that indicates if the node belongs to $X$.
We show that nested \wmsoup automata are closed under the three kinds of quantifier of \wmsoup logic, with the quantifiers encoded using $\otimes$ as follows:
	\begin{eqnarray*}
		\exists_{\mathrm{fin}} X L  &\eqdef& \set{t : t \otimes X \in L \mbox{ for some finite set of nodes $X$}}\\
		\exists_{\mathrm{path}} \pi L  &\eqdef& \set{t : t \otimes \pi \in L \mbox{  for some path $\pi$}}\\
		\mathsf U_{\mathrm{chain}} X L  &\eqdef& \set{t :t \otimes X \in L \mbox{  for  arbitrarily large finite chains $X$} }.
	\end{eqnarray*}
	
% Recall the notation $t \otimes X$ introduced 
% 
% We now show that the languages recognized by nested automata are
% closed under the three types of quantification that are allowed in \wmsoup.
% Therefore, to complete the logic-to-automata proof of Theorem~\ref{thm:equal-to-nested}, it suffices to prove the following lemma.


		



\subsubsection{Closure under weak existential quantification}
  An equivalence relation on trees is called a \emph{tree congruence} if for every tree that has more than one node, its equivalence class is uniquely determined by its root label and the equivalence classes of the subtrees rooted in the left and right children of the root.
  An equivalence relation is said to \emph{saturate} a  set if the set is a union of equivalence classes.

\begin{lemma}\label{lem:a-congruence}
	Let $\Aa$ be a nested \wmsoup automaton. There is a tree congruence which saturates the language of $\Aa$, and  such that every equivalence class is recognised by some nested \wmsoup automaton.
\end{lemma}
\begin{mproof}
	Induction on the nesting depth. 
	

		
			Consider a nested \wmsoup automaton $\Aa$. Let $\Aa_0$ be its main automaton, and be $\Aa_1,\ldots,\Aa_k$ the lookahead automata.  	 	We only prove the lemma for the case when the main automaton of $\Aa$ is an atomic counter automaton. 
 For every state $q$ of the transducer in the main automaton, let $\Aa^q$ be the same nested automaton as $\Aa$, except that the initial state of the transducer in the main automaton is changed to $q$.
	

		Let us recall the semantics of a nested automaton, as applied to  the nested automaton $\Aa^q$. Given an input tree, the automaton begins by producing the tree 
	\begin{align}
		t[\Aa_1,\ldots,\Aa_k]  \label{eq:intermediate-tree-in-nested-semantics}.
	\end{align}
	Based on the root label of this  tree and the initial state $q$, the transducer in the main automaton sends states $q_0$ and $q_1$ to the  left and right subtrees $t|_0$ and $t|_1$.  The nested automaton $\Aa^q$ accepts $t$ if and only if for every $i \in \set{0,1}$, the automaton  $\Aa^{q_i}$ accepts  subtree $t|_i$.

	
	For every $i \in \set{1,\ldots,k}$, the induction assumption gives  a tree congruence $\sim_i$ which saturates the language recognised by the lookahead automaton $\Aa_i$. 	
 Let $\sim_0$ be the  equivalence relation which considers two trees equivalent if they are accepted by the same automata $\Aa^q$, ranging over all states $q$ of the transducer. Clearly this relation saturates the language of every $\Aa^q$, in particular it saturates the language of $\Aa$.  Let $\sim$ be the intersection of $\sim_i$ ranging over all $i \in \set{0,\ldots,k}$.  We claim that this is a tree congruence.
 
 
 Let then $t$ and $t'$ be trees that  have the same root label, and such that for every child number $i \in \set{0,1}$, the subtrees $t|_i$ and $t'|_i$ are $\sim$-equivalent. We need to show that $t$ and $t'$ are $\sim$-equivalent.
Because $\sim$ refines the  equivalences $\sim_1,\ldots,\sim_k$, and these are tree congruences, it follows that $t$ and $t'$ are $\sim_i$-equivalent  for every $i \in \set{1,\ldots,k}$. It remains to prove $t \sim_0 t'$, which says that for every state $q$ of the transducer in the main automaton of $\Aa$, the automaton $\Aa^q$ accepts both, or rejects both, of the trees $t$ and $t'$. By the assumption that $t \sim_i t'$ holds for every $i \in \set{1,\ldots,k}$, it follows that the trees
	\begin{align*}
		t[\Aa_1,\ldots,\Aa_k] \qquad \mbox{and}\qquad 		t'[\Aa_1,\ldots,\Aa_k]
	\end{align*}
	have the same root labels. In particular, the states $q_0$ and $q_1$, as discussed in the paragraph after~\eqref{eq:intermediate-tree-in-nested-semantics}, are the same for both $t$ and $t'$. The result then follows by the  assumption that $t|_0 \sim_0 t'|_0$ and  $t|_1 \sim_0 t'|_1$.
\end{mproof}

We use the name \emph{$\Aa$-congruence} for the congruence described in the above lemma, and the name \emph{$\Aa$-type} for the equivalence classes. We write $t_{/\Aa}$ for the $\Aa$-type of a tree $t$. Since nested \wmsoup are closed under finite unions, the following lemma implies that languages recognised by nested automata are closed under weak existential quantification $L \mapsto \exists_{\mathrm{fin}}X L$.

\begin{lemma}\label{lem:a-congruence-projection}
	Let $\Aa$ be a nested \wmsoup automaton with input alphabet $A \times \set{0,1}$. For every $\Aa$-type  $\tau$, there is a nested \wmsoup automaton recognising the set 
	\begin{align*} 
		\set{ t : \mbox{for some finite set $X$, the $\Aa$-type of $t \otimes X$ is $\tau$}} \subseteq \trees A
	\end{align*}
\end{lemma}
\begin{mproof}
	By Lemma~\ref{lem:a-congruence}, for every $\Aa$-type $\tau$, the set of trees with $\Aa$-type $\tau$ is recognised by a nested \wmsoup automaton. 
Consider the relabeling 
\begin{align*}
	f : A \times A \to \set{0,1}  \qquad\mbox{defined by}\qquad  f(a)=(a,0).
\end{align*}
Langauges recognised by nested \wmsoup automata are easily seen to be closed under inverse images of relabelings and therefore for every $\Aa$-type $\tau$, the  set 
	\begin{align*}
		\set { t  : t \otimes \emptyset \mbox{ has $\Aa$-type $\tau$ }} = f^{-1}(\tau)
	\end{align*}
	is recognised by a nested \wmsoup automaton, call it $\Aa_\tau$.
	
	 The automaton for the language in the statement of the lemma works as follows. Its lookahead automata are the automata $\Aa_\tau$, ranging over all $\Aa$-types, let these lookahead automata be $\Aa_1,\ldots,\Aa_k$. Its main automaton is an atomic prefix automaton.  It is not difficult to see that if $X$ is a finite set of nodes in a tree $t$ over the alphabet $A$, then the  $\Aa$-type of the tree $t \otimes X$ is uniquely determined by the labels of those (finitely many) nodes in 
	 \begin{align*}
	 	t[\Aa_1,\ldots,\Aa_k] \otimes X
	 \end{align*}
	 which have descendants in $X$. Indeed, for a node $x$ that has no descendants (including itself) in $X$,   the lookahead  automata give the $\Aa$-type of the subtree
	\begin{align*}
		(t \otimes X)|_{x} = t|_{x} \otimes \emptyset.
	\end{align*}
	For nodes that have descendants in $X$, the tree congruence yields a multiplication table that  can be used to compute their $\Aa$-types. This multiplication table can be implemented by a finite state device as in the main automaton.
\end{mproof}

\subsubsection{Closure under chain unbounding quantification}
In this section we show Lemma~\ref{lem:closed-under-unbounding-chain}, which shows that languages recognised by nested \wmsoup automata are closed under  chain unbounding quantification.

\begin{lemma}\label{lem:closed-under-unbounding-chain}
	For every  nested \wmsoup automaton $\Aa$, the language 
	\begin{align*}
	\mathsf U_{\mathrm{chain}} X \Aa  \eqdef 	\set{ t : \mbox{ $t \otimes X$ is accepted by $\Aa$ for arbitrarily large finite chains $X$}}
	\end{align*}
	is also recognised by a nested \wmsoup automaton.
\end{lemma}
Before proving the lemma, we state and prove Lemmas~\ref{lem:counter-tree-has-good-properties-for-unbounding} and~\ref{lem:counter-tree-t-can-be-produced}.

Let $\Aa$ be a nested \wmsoup automaton recognising the language $L$, whose input alphabet is $A \times \set{0,1}$. We use the notion of $\Aa$-types as in the previous section, i.e.~$\Aa$-types are equivalence classes of a tree congruence obtained by applying Lemma~\ref{lem:a-congruence} to $\Aa$.
	Given a tree $t$ over  alphabet $A$, define a  counter tree
	\begin{align*}
		[t]  \in \countertrees{\mbox{types($\Aa$)}}
	\end{align*}
	where the counters are $\Aa$-types, as follows.  
	The nodes of $[t]$ are the same as the nodes of $t$. 
	For a node $x$ in a tree $t$,
	define an $x$-chain to be a chain which does not contain the sibling of $x$, nor any of its descendants. Equivalently, an $x$-chain is a chain that is contained in some path that passes through $x$.
	 For a node $x$ and its parent $y$, and $\Aa$-types $\tau$ and $\sigma$, the counter tree $[t]$ contains  an  edge  
	 \begin{align*}
(x,\tau) \to (y,\sigma)
	 \end{align*} if there exists a finite $x$-chain $X$ such that:
	\begin{itemize}
		\item 	 $t \otimes X$ is accepted by $\Aa$;
		\item  the $\Aa$-type $(t \otimes X)|_{x}$ is $\tau$ 
		\item  the $\Aa$-type of $(t \otimes X)|_{y}$ is $\sigma$.
	\end{itemize}
	 The edge is labelled by ``increment'' if $X$ contains $x$, otherwise it is labelled by ``transfer''.  Note that the edges in this counter tree are directed toward the root.



\begin{lemma}\label{lem:counter-tree-has-good-properties-for-unbounding}
A tree $t$ belongs to $\mathsf U_{\mathrm{chain}} X L$ 	 if and only if on some path, some counter in $[t]$ is tail unbounded.\end{lemma}
\begin{mproof}
	From the definition of the counter tree $[t]$ it is not  difficult to see that  the following conditions are equivalent:
	\begin{enumerate}
		\item $t \otimes X \in L$ holds for some finite chain $X$ of size at least $n$;
		\item some counter in some node of $[t]$ has value at least $n$.
	\end{enumerate}
Another property of the counter tree $[t]$ is that if in a node $x$ some counter has value at least $n$ then: 
\begin{enumerate}
	\item[a.]  in the parent of $x$ some counter  has value at least $n$;
	\item[b.] in some child of $x$ some  counter has value at least $n-1$
\end{enumerate}
By item a.~and the equivalence of 1 and 2, a tree belongs to $\mathsf U_{\mathrm{chain}} X L$ if and only if in the root of the counter tree $[t]$, some counter has value $\infty$. By item b., if in some node $x$, some counter has value $\infty$, then the same is true in some child of $x$. Therefore, for a tree $t$ we have two cases:
\begin{itemize}
	\item If $t$ belongs to $\mathsf U_{\mathrm{chain}} X L$, then on some  infinite path, in every node some counter has value $\infty$. In particular, on some infinite path some counter is tail unbounded.
	\item Otherwise, there is a finite upper bound on the values of all counters in the whole tree, in particular on every path every counter is not tail unbounded.
\end{itemize} 
\end{mproof}

Define a  \emph{nested \wmsoup transducer} with input alphabet $A$ and output alphabet $B$ as follows. It consists of finitely many nested \wmsoup automata $\Aa_1,\ldots,\Aa_k$ over the input alphabet $A$, call them the \emph{lookahead automata}, and a deterministic transducer $f$ with input alphabet $A \times \set{0,1}^k$ and output alphabet $B$. The function defined by the transducer is 
\begin{align*}
	t \in \trees A \qquad \mapsto \qquad f(t[\Aa_1,\ldots,\Aa_k]) \in \trees B
\end{align*}

\begin{lemma}\label{lem:composing-transducer-with-automaton}
	If $f$ is recognised by a nested \wmsoup transducer, and $L$ is recognised by a nested \wmsoup automaton, then $f^{-1}(L)$ is recognised by a nested \wmsoup automaton.
\end{lemma}
\begin{mproof}
	By composing the transducer with the automaton.
\end{mproof}

The following lemma shows that the counter tree $[t]$ can be produced by a deterministic transducer which has access to information produced by nested \wmsoup automata.
\begin{lemma}\label{lem:counter-tree-t-can-be-produced} The function $t \mapsto [t]$ is recognised by a nested \wmsoup transducer. 
\end{lemma}
\begin{mproof}
	By Lemma~\ref{lem:a-congruence}, for every $\Aa$-type $\tau$, there is a nested \wmsoup automaton $\Aa_\tau$ that recognises $\tau$. Using these automata, 
	 it is not difficult to show that  for every child of the root $x \in \set{0,1}$ and $\Aa$-types $\tau,\sigma$, there is a nested \wmsoup automaton, call it $\Aa_{\tau,x,\sigma}$, which accepts a tree $t$ over the alphabet $A$ if and only if there is some finite  $x$-chain $X$ such that  the $\Aa$-type of $t \otimes X$ is $\tau$ and the $\Aa$-type of the subtree $(t \otimes X) |_x$ is $\sigma$.
	 The finitely many automata in the statement of the lemma are the automata $\Aa_{\tau,x,\sigma}$, for all possible values of $\tau$, $x$ and $\sigma$. The transducer  simply implements the definition of the counter tree $[t]$. The only nontrivial issue is that it needs to keep track, for every node $x$, of the set 
	 \begin{align*}
	 	\set{\tau : t \otimes X \in L \mbox{ holds for some finite $x$-chain $X$ with $(t \otimes X)|_x$ having $\Aa$-type $\tau$}}.
	 \end{align*}
	 This set can be stored and updated using the finite control of the transducer.
\end{mproof}

\begin{mproof}[of Lemma~\ref{lem:closed-under-unbounding-chain}] 
	By Example~\ref{ex:boolean-nesting},  nested \wmsoup automata are closed under complement.
	Therefore, it suffices to  give a nested \wmsoup  automaton for the complement of the language in Lemma~\ref{lem:closed-under-unbounding-chain}, i.e.~for the set of trees $t$ where there is a bound on the size of chains $X$ such that $\Aa$ accepts $t \otimes X$.  
	 By Lemma~\ref{lem:counter-tree-has-good-properties-for-unbounding}, a tree does not belong to the language from Lemma~\ref{lem:closed-under-unbounding-chain}  if and only if in the counter tree $[t]$, all counters are tail bounded on all paths. Testing if all counter all tail bounded on all paths can be done by an atomic counter automaton, while the tree $[t]$ can be computed by a nested \wmsoup transducer thanks to  Lemma~\ref{lem:counter-tree-t-can-be-produced}. The result follows by Lemma~\ref{lem:composing-transducer-with-automaton}.
\end{mproof}


 
 \begin{align*}
 	downloop_t(x,c,d,i)
 \end{align*}
 For a counter tree $t$ over counters $C$, define the weighted tree
 \begin{align*}
 	down(t) \in \trees{\bar \Nat^{C \times C \times \set{0,1}}}
 \end{align*}
 to be the tree where the vector stored in 
 
 \begin{lemma}\label{lem:move-up-the-downvalue}
	 For every  \wmsoup transducer 
 \begin{align*}
 	f : \trees A \to \countertrees C
 \end{align*}
 the there exists a \wmsoup transducer representing the  function
 \begin{align*}
 	t \in \trees A \qquad \mapsto \qquad side_f(t) \in \trees {A \times \bar \Nat^{C^2}}.
 \end{align*} 	
 \end{lemma}


\begin{lemma}\label{lem:}
   	 For every  \wmsoup transducer 
    \begin{align*}
    	f : \trees A \to \countertrees C
    \end{align*} and family $\Uu$ of subsets of $C$, there exists a formula $\varphi$ of weighted \wmsou, with label alpahbet $A$ and weight alphabet $C^2$, such that for every tree $t$ over alphabet $A$ and every full path $\pi$,  the following conditions are equivalent
	\begin{itemize}
		\item the $\Uu$-acceptance condition is satisfied by $\pi$ in $f(t)$; 
		\item the path-word $side_f(t) \restrict \pi$ satisfies $\varphi$
	\end{itemize}
\end{lemma}
 \begin{lemma}\label{lem:move-up-the-downvalue}
For every \wmsoup transducer 
 \begin{align*}
 	f : \trees {A \times \set{0,1}} \to \countertrees C
 \end{align*}
 and a family $\Uu$ of subsets of $C$, there exists a \wmsoup transducer 
 \begin{align*}
   \hat f : \trees A \to \trees {\set{accept,reject}}
 \end{align*}
 such that for every tree $t$ over $A$, and  every full paths $\pi$, and every node $x \in \pi$ the following conditions are equivalent:
 \begin{itemize}
 	\item In  the counter tree $f(t \otimes \pi)$, the  $\Uu$-acceptance condition is satisfied by every  full path $\sigma \neq \pi$ such that $x$ is the maximal node in the intersection $\pi \cap \sigma$.
\item The label of node $x$ in $\hat f(t)$ is $yes$.
 \end{itemize}
 \end{lemma}
 
  \begin{lemma}\label{lem:move-up-the-downvalue}
 For every \wmsoup transducer 
  \begin{align*}
  	f : \trees {A \times \set{0,1}} \to \countertrees C
  \end{align*}
  and a family $\Uu$ of subsets of $C$, there exists a nested \wmsoup automaton $\Aa$  with input alphabet $A$  which accepts a tree $t$ if and only if for every full path $\pi$, the $\Uu$-acceptance condition is satisfied by $\pi$ in $f(t \otimes \pi)$. 
  \end{lemma}
 
 
  \begin{lemma}\label{lem:move-up-the-downvalue}
 For every \wmsoup transducer 
  \begin{align*}
  	f : \trees {A \times \set{0,1}} \to \countertrees C
  \end{align*}
  and a family $\Uu$ of subsets of $C$, there exists a nested \wmsoup automaton 
 $\Aa$ with input alphabet $A  \times \set{0,1}$, such that for every tree $t$ over alphabet $A$ and node $x$ in $t$, the following conditions are equivalent:
  \begin{itemize}
  	\item $\Aa$ accepts $t \otimes \set{x}$,
	\item for every paths $\pi \neq \sigma$ such that $x$ is the maximal node in the intersection $\pi \cap \sigma$, the $\Uu$-acceptance condition is satisfied by $\sigma$ in  $f(t \otimes \pi)$.
  \end{itemize}
  
   $\Aa$ accepts a tree 
  $t \otimes \set{x}$ if and only if for every paths $\pi \neq \sigma$
   nested \wmsoup automata $\Aa_{=}$ and $\Aa_{\neq}$ with input alphabet $A$  such that for every tree $t$ over $A$:
  \begin{enumerate}
     	\item $\Aa_=$ accepts   $t$ if and only if for every full path $\pi$, the $\Uu$-acceptance condition is satisfied by $\pi$ in $f(t \otimes \pi)$.  
  	\item $\Aa_{\neq}$ accepts   $t$ if and only if for every full paths $\pi \neq \sigma$, the $\Uu$-acceptance condition is satisfied by $\sigma$ in $f(t \otimes \pi)$.  
  \end{enumerate}
  \end{lemma}
 
 
 \begin{lemma}\label{lem:}
 	Consider a nested \wmsoup automaton $\Aa$ with input alphabet $A$. There exists a nested \wmsoup transducer 
	\begin{align*}
		f : \trees A  \to \trees {P(\set{0,1})}
	\end{align*}
	such that for every tree $t$ over $A$ and every infinite path $\pi$, the label 
 \end{lemma}
 \begin{lemma}\label{lem:}
 	Consider a \wmsoup transducer
	\begin{align*}
		f : \trees {A \times \set{0,1}} \to \countertrees C.
	\end{align*}
	and a family $\Uu$ of subsets of $C$. There is a formula 
	For every $c \in C$ there exists a formula  such that for every tree $t$ over $A$ and every  path $\pi$ in $t$, 
	\begin{itemize}
		\item the 
	\end{itemize}
 \end{lemma}
 
 \begin{lemma}\label{lem:}
 	For every nested \wmsoup automaton $\Aa$ with input alphabet $A \times \set{0,1}$, there are finite sets $A',C$,  nested \wmsoup transducers
	\begin{align*} 
	f : \trees A \to \trees {A'}  	\qquad g : \trees A \to \countertrees {B}
	\end{align*}
	and a formula $\varphi$ of weighted \wmsou with label alphabet $A'$ and weight alphabet $B$  such that
	\begin{align*}
		\mbox{$\Aa$ accepts }t \otimes \pi \qquad \mbox{iff} \qquad f(t) \otimes val_{g(t)} \restrict \pi \models \varphi	\end{align*}
	holds for every tree $t$ over alphabet $A$ and every full path $\pi$ in $t$.
	 \end{lemma}
\begin{mproof}
	
The proof is by induction on the nesting depth of the automaton $\Aa$. Suppose that the main automaton in $\Aa$ is $\Aa_0$ and the lookahead automata are $\Aa_1,\ldots,\Aa_k$. We only consider the more interesting case when the main automaton $\Aa_0$ is an atomic counter automaton. 

Let $C$ be the counters of $\Aa_0$. For a counter tree  $t$, define the the \emph{down-value} of a counter pair $(c,d) \in C^2$ in  a node $x$, denoted by 
\begin{align*}
	downval_{t}(x,c,d)  \in \bar \Nat,
\end{align*}
to be the least upper bound on the number of increments that can be found on a counter path that begins in node $x$ and counter $c$, ends in node $x$ and counter $d$, and only visits nodes in the subtree of $x$. Using a standard method of converting two-way tree automata to one-way tree automata, see e.g.~\cite{DBLP:conf/icalp/Vardi98}, one can show that the down-values can be computed by  a deterministic transducer 
\begin{align*}
	\gamma : \countertrees C \to \countertrees {C^2}
\end{align*}
in the sense that for every counter tree $t$ over counter $C$, 
\begin{align*}
val_{\gamma(t)}(x,(c,d)) = 	downval_t(x,c,d)  \qquad \mbox{for every node $x$ and counter $c,d$}.
\end{align*}

\begin{align*}
	\delta_q : \trees A \to \countertrees {C^2}
\end{align*}
such that for every tree $t$ over alphabet $A$ and every node $x$, 
\begin{align*}
	val_{\delta_q(t)}(x,(c,d)) = downval(f_q(t|_x[\Aa_1,\ldots,\Aa_k]),c,d)
\end{align*}

\begin{align*}
	val_{\delta_{qi}(t)}(x,(c,d)) = downval(f_q(t|_{xi}[\Aa_1,\ldots,\Aa_k]),c,d)
\end{align*}


 For every $i \in \set{1,\ldots,k}$,  apply the induction assumption to the lookahead automaton $\Aa_i$,  yielding 
	\begin{align*} 
	A'_i, B_i, f_i,g_i,\varphi_i
	\end{align*}
s

\end{mproof} 



<<<<<<< Local Changes
<<<<<<< Local Changes
From the above two lemmas, we obtain closure of languages recognised by nested \wmsoup automata under universal path quantification.

\subsection{Tail bounded}
\subsubsection{Tail unbounded.} For some constructions, it is convenient to have an acceptance condition that is prefix independent. If $t$ is a counter tree with counters $C$, and $c \in C$, then the condition 
\begin{align*}
	\limsup_{x \in \pi} \val_t(x,c)  = \infty \qquad \mbox{for every path $\pi$}
\end{align*}
is not prefix independent in the sense that changing a single label in $t$ could  change the truth value, as shown in the following example.

\begin{example}\label{ex:not-prefix-independent}
	Consider a counter tree $t$ with counters $\set{c,d}$. Let the counter operations be defined so that counter $d$ has value $\infty$ in the root node, e.g.~on every  node of the leftmost path transfers counter $d$ with an increment to counter $d$ in its parent.	
	For counter $c$, we assume that for every node $x$ and its child $y$, there is an edge which transfers $c$ in $x$ to $c$ in $y$ without an increment. In this tree, there is no connection between counters $c$ and $d$, and there are no increments on counter $c$, and therefore $c$ has value $0$ in every node. However, if we change the root so that counter $d$ in the root is transferred to counter $c$  in the root, then in the resulting counter tree, call it $t'$, counter $c$ has value $\infty$ in every node.
\end{example}

To achieve prefix independence, we use the following definition: counter $c$ is  \emph{tail unbounded} on a path $\pi$ in a counter tree $t$ if $\pi$  if   $c$ is unbounded on  $\pi$ in every counter tree $t'$  that agrees with $t$ on all but finitely many nodes. 

\begin{example}
	In Example~\ref{ex:not-prefix-independent}, counter $d$ is tail unbounded on the leftmost path in both $t$ and $t'$. Counter $c$ is not tail unbounded on any path, in either of these trees. 
\end{example}=======
From the above two lemmas, we obtain closure of languages recognised by nested \wmsoup automata under universal path quantification.

		
		
		By Lemma, there exists an atomic counter language $K$ such that 
		\begin{align*}
			g(t \otimes X)  \restrict \pi \models \psi \qquad \mbox{for every full path $\pi$}
		\end{align*}
		holds if and only if 
		\begin{align*}
			g(t \otimes X) \in L
		\end{align*}
		
	\begin{lemma}\label{lem:}
		There exists a formula $\varphi$ of weighted \wmsou such that for every tree $t$ over alphabet $A$, a  full path $\pi$ in $t$  is $\Uu$-accepting in $f(t)$ if and only if
			\begin{align*}
				\sidevalue_f(t) \otimes t \restrict \pi \models \varphi
			\end{align*}
	\end{lemma}
	\begin{mproof}
	Applying   Lemma~\ref{lem:counter-unbounded-separation} to all counters in $C$ and using a Boolean combination,  we get a formula as in the statement of the lemma, except that  instead of $\sidevalue_f(t) \otimes t \restrict \pi$  we have  $\sidevalue_f(t) \otimes f(t) \restrict \pi$. Since $f(t)$ does not use lookahead, the values of $f(t)$ on the path $\pi$ can be computed, using weak quantification, based only on the path $\sidevalue_f(t) \otimes t$. 
	\end{mproof}
	
	\begin{lemma}\label{lem:}
		There exists a formula of $\varphi$ of weighted \wmsou such that for every tree $t$ and every full path $\pi$ in $t$, 
		\begin{align}
			t \otimes X \otimes \sidevalue_f(t) \models \varphi
		\end{align}
holds if and only if $f(t|_x) \in L$ holds for every node $x \in X$.
	\end{lemma}


	
	  every node $x$ in $t$ and every path $\pi$ in the subtree $t|_x$, the following conditions are equivalent:
		\begin{itemize}
			\item counter $c$ is tail unbounded on path $\pi$ in $f(t|_x)$.
						\item $\varphi$ is true in $(\sidevalue_f(t) \otimes t)|_x \restrict \pi$;
		\end{itemize}

for every counter $c \in C$, there exists a formula $\varphi_c$ of weighted \wmsoup  such that for every path $\pi$ in $t$, counter $c$ is tail unbounded on path $\pi$ in $f(t)$ if and only if 
		 	\begin{align*}
		  \sidevalue_f(t) \otimes t \restrict \pi \models \varphi_c.
		 	\end{align*}
By modifying this formula $\varphi_c$, one can define a formula $\varphi_c(x)$ with one free variable, such that for every full path $\pi$ in $t$ and every node $x \in \pi$,  counter $c$ is tail unbounded on path $\pi$ in $f(t|_x)$ if and only if 
	


\begin{lemma}\label{lem:}
	For every $f$ and $L$ as in~\ref{lem:characteristic-function-in-wmsoup-automata} there exists a deterministic transducer without lookahead 
	\begin{align*}
		g : \trees {A \times 2} \to \countertrees \Sigma
	\end{align*}
	and a formula $\varphi$ of weighted \wmsou with input alphabet $\Sigma$ such that the characteristic language of $f^{-1}(L)$ is 
	\begin{align}
		\set{t \otimes X :  g(t) \restrict \pi \models \varphi \mbox{ for every full path in $t$}}
	\end{align}
\end{lemma}
The rest of Section~\ref{sec:from-nested-to-inf-sup} is devoted to showing the above lemma. Let $f$ and $L$ be as in the lemma. 


In other words, we need to show that 	if $L$ is an atomic counter language, then both the languages
	\begin{align}\label{eq:subtrees-labelled-languages-all-paths}
		\set{t \otimes X : \mbox{ $t|_x \in L$ for every $x \in X$}}\\
	\label{eq:subtrees-labelled-languages-not-some-path}			\set{t \otimes X : \mbox{$t|_x \not \in L$ for every $x \in X$}}
	\end{align}
	are recognised by  \wmsoup automata. The rest of Section~\ref{sec:from-nested-to-inf-sup} is devoted to proving this.

The proof strategy is as follows. In Section~\ref{sec:for-all-nondeterministic}, we  show that the langauges in the statement of the lemma are recognised by  nondeterministic atomic counter automata. Then, in Section~\ref{sec:nondeterministic-to-inf-sup} we show that every nondeterministic atomic counter automaton can be simulated by a flat \wmsoup automaton.





\subsection{Nondeterministic atomic counter automata}
\label{sec:for-all-nondeterministic}
Define a \emph{nondeterministic atomic counter automaton} to be like an atomic counter automaton, except that the transducer is nondeterministic. In other words, these automata recognise projections of languages recognised by atomic counter automata.  The goal of this section is to prove the following lemma.

\begin{lemma}\label{lem:for-all-at-cost-of-nondeterminism}
	Let $\Aa$ be an  atomic counter automaton. Then both the languages
	\begin{eqnarray*}
		\set{t \otimes X : \mbox{$\Aa$ accepts the subtree $t|_x$ for every $x \in X$}}\\
				\set{t \otimes X : \mbox{$\Aa$ rejects the subtree $t|_x$ for every $x \in X$}}
	\end{eqnarray*}
	are recognised by nondeterministic atomic counter automata.
\end{lemma}

Actually, nondeterminism is only used for the second language.
We begin with the following lemma, which is the converse of Lemma~\ref{lem:weighted-on-all-paths}.
\begin{lemma}\label{lem:atomic-to-weighted-reading-down}
	For every atomic counter automaton $\Aa$ over alphabet $A$ there is a deterministic transducer
	transducer
	\begin{align*}
		f : \trees A \to \countertrees C
	\end{align*}
	that produces only down counter trees, and a formula $\varphi$ of weighted \mso, such that  $\Aa$ accepts a tree $t$ if and only if every full path $\pi$ satisfies
	\begin{align*}
		f(t)\restrict \pi \models \varphi.
	\end{align*}
\end{lemma}
\begin{mproof}
	\begin{center}
		(TODO estimated at one paragraph)
	\end{center}
\end{mproof}








\begin{lemma}\label{lem:tape-down}
	Let 
	\begin{align*}
		f: \trees A \to \countertrees C 
	\end{align*}
	be a deterministic transducer, which  produces only down counter trees. There is a finite set $B$ and deterministic transducers
	\begin{align*}
		g : \trees A \to \countertrees {C \times B}\\
		h : \trees A \to \trees B
	\end{align*}
	such that for every tree $t \in \trees A$ and nodes $x \le xy$, if $b \in B$ is the label of $x$ in $h(t)$, then
	\begin{align*}
		val_{f(t|_x)}(c,y)  = val_{g(t)}((c,b),xy)
	\end{align*}
\end{lemma}
\begin{mproof}
	(TODO tape construction, estimated at 5 paragraphs)
\end{mproof}



We now establish the first part of Lemma~\ref{lem:for-all-at-cost-of-nondeterminism}, not that we do not use nondeterminism here.
\begin{lemma}\label{lem:every-subtree-is-actually-atomic}
If  $\Aa$ is an atomic counter automaton, then
\begin{align*}
			\set{t \otimes X : \mbox{$\Aa$ accepts the subtree $t|_x$ for every $x \in X$}}
\end{align*}
is recognised by an atomic counter automaton.
\end{lemma}
\begin{mproof}
	Apply Lemma~\ref{lem:atomic-to-weighted-reading-down} to $\Aa$, yielding a transducer 
	\begin{align*}
		f : \trees A \to \countertrees C
	\end{align*}
	and a formula $\varphi$ of weighted \wmso+u+u. By the lemma, a subtree $t|_x$ is accepted by $\Aa$ if and only if for every full path $\pi$ in the subtree $t|_x$, 
	\begin{align}\label{eq:weighted-formula-on-a-path}
		val_{f(t|_x)} \restrict \pi \models \varphi.
	\end{align}
	Apply Lemma~\ref{lem:tape-down} to the transducer $f$, yielding transducers $g$ and $h$. For $b \in B$, define $\varphi_b$ to be like $\varphi$, except that instead of reading counter $c$, it reads counter $(c,b)$. By Lemma~\ref{lem:tape-down} we know that if the label of node $x$ in the tree $h(t)$ is $b$, then~\eqref{eq:weighted-formula-on-a-path} is equivalent to
	\begin{align*}
		val_{g(t)} \restrict x\pi \models \varphi_b,
	\end{align*}
	where $x\pi$ is the path obtained by shifting $\pi$ so that its first node becomes $x$. It follows that there is a formula $\psi$ of weighted \wmso+u+u such that for every infinite path $\pi$, not necessarily beginning in the root, we have 
	\begin{align*}
		val_{f(t|_x)} \restrict \pi \models \varphi \qquad \mbox{iff} \qquad h(t) \otimes val_{g(t)} \restrict x\pi \models \psi.
	\end{align*}
	Define $\psi'$ to be the formula which is true in a word 
	\begin{align*}
		w \otimes v \qquad \mbox{with } w\in  (B \times \bar \Nat^{C})^\omega \mbox{ and } v \in  \set{0,1}^\omega
	\end{align*}	
	if $\psi$ is true in every suffix of $w$ that begins with a position that has label $1$ in $v$. This is also a formula of weighted \wmso+u+u. By the properties of $\psi$, it follows that  a tree $t \otimes X$ belongs to the language from the statement of the lemma if and only if $\psi'$ is true in every path of the tree
	\begin{align*}
		h(t) \otimes val_{g(t)} \otimes X.
	\end{align*}
	Therefore, by Lemma~\ref{lem:weighted-on-all-paths}, the language in the statement of the lemma is recognised by an atomic counter automaton.	
\end{mproof}

>>>>>>> External Changes
=======
From the above two lemmas, we obtain closure of languages recognised by nested \wmsoup automata under universal path quantification.

		
		
		By Lemma, there exists an atomic counter language $K$ such that 
		\begin{align*}
			g(t \otimes X)  \restrict \pi \models \psi \qquad \mbox{for every full path $\pi$}
		\end{align*}
		holds if and only if 
		\begin{align*}
			g(t \otimes X) \in L
		\end{align*}
		
	\begin{lemma}\label{lem:}
		There exists a formula $\varphi$ of weighted \wmsou such that for every tree $t$ over alphabet $A$, a  full path $\pi$ in $t$  is $\Uu$-accepting in $f(t)$ if and only if
			\begin{align*}
				\sidevalue_f(t) \otimes t \restrict \pi \models \varphi
			\end{align*}
	\end{lemma}
	\begin{mproof}
	Applying   Lemma~\ref{lem:counter-unbounded-separation} to all counters in $C$ and using a Boolean combination,  we get a formula as in the statement of the lemma, except that  instead of $\sidevalue_f(t) \otimes t \restrict \pi$  we have  $\sidevalue_f(t) \otimes f(t) \restrict \pi$. Since $f(t)$ does not use lookahead, the values of $f(t)$ on the path $\pi$ can be computed, using weak quantification, based only on the path $\sidevalue_f(t) \otimes t$. 
	\end{mproof}
	
	\begin{lemma}\label{lem:}
		There exists a formula of $\varphi$ of weighted \wmsou such that for every tree $t$ and every full path $\pi$ in $t$, 
		\begin{align}
			t \otimes X \otimes \sidevalue_f(t) \models \varphi
		\end{align}
holds if and only if $f(t|_x) \in L$ holds for every node $x \in X$.
	\end{lemma}


	
	  every node $x$ in $t$ and every path $\pi$ in the subtree $t|_x$, the following conditions are equivalent:
		\begin{itemize}
			\item counter $c$ is tail unbounded on path $\pi$ in $f(t|_x)$.
						\item $\varphi$ is true in $(\sidevalue_f(t) \otimes t)|_x \restrict \pi$;
		\end{itemize}

for every counter $c \in C$, there exists a formula $\varphi_c$ of weighted \wmsoup  such that for every path $\pi$ in $t$, counter $c$ is tail unbounded on path $\pi$ in $f(t)$ if and only if 
		 	\begin{align*}
		  \sidevalue_f(t) \otimes t \restrict \pi \models \varphi_c.
		 	\end{align*}
By modifying this formula $\varphi_c$, one can define a formula $\varphi_c(x)$ with one free variable, such that for every full path $\pi$ in $t$ and every node $x \in \pi$,  counter $c$ is tail unbounded on path $\pi$ in $f(t|_x)$ if and only if 
	


\begin{lemma}\label{lem:}
	For every $f$ and $L$ as in~\ref{lem:characteristic-function-in-wmsoup-automata} there exists a deterministic transducer without lookahead 
	\begin{align*}
		g : \trees {A \times 2} \to \countertrees \Sigma
	\end{align*}
	and a formula $\varphi$ of weighted \wmsou with input alphabet $\Sigma$ such that the characteristic language of $f^{-1}(L)$ is 
	\begin{align}
		\set{t \otimes X :  g(t) \restrict \pi \models \varphi \mbox{ for every full path in $t$}}
	\end{align}
\end{lemma}
The rest of Section~\ref{sec:from-nested-to-inf-sup} is devoted to showing the above lemma. Let $f$ and $L$ be as in the lemma. 


In other words, we need to show that 	if $L$ is an atomic counter language, then both the languages
	\begin{align}\label{eq:subtrees-labelled-languages-all-paths}
		\set{t \otimes X : \mbox{ $t|_x \in L$ for every $x \in X$}}\\
	\label{eq:subtrees-labelled-languages-not-some-path}			\set{t \otimes X : \mbox{$t|_x \not \in L$ for every $x \in X$}}
	\end{align}
	are recognised by  \wmsoup automata. The rest of Section~\ref{sec:from-nested-to-inf-sup} is devoted to proving this.

The proof strategy is as follows. In Section~\ref{sec:for-all-nondeterministic}, we  show that the langauges in the statement of the lemma are recognised by  nondeterministic atomic counter automata. Then, in Section~\ref{sec:nondeterministic-to-inf-sup} we show that every nondeterministic atomic counter automaton can be simulated by a flat \wmsoup automaton.





\subsection{Nondeterministic atomic counter automata}
\label{sec:for-all-nondeterministic}
Define a \emph{nondeterministic atomic counter automaton} to be like an atomic counter automaton, except that the transducer is nondeterministic. In other words, these automata recognise projections of languages recognised by atomic counter automata.  The goal of this section is to prove the following lemma.

\begin{lemma}\label{lem:for-all-at-cost-of-nondeterminism}
	Let $\Aa$ be an  atomic counter automaton. Then both the languages
	\begin{eqnarray*}
		\set{t \otimes X : \mbox{$\Aa$ accepts the subtree $t|_x$ for every $x \in X$}}\\
				\set{t \otimes X : \mbox{$\Aa$ rejects the subtree $t|_x$ for every $x \in X$}}
	\end{eqnarray*}
	are recognised by nondeterministic atomic counter automata.
\end{lemma}

Actually, nondeterminism is only used for the second language.
We begin with the following lemma, which is the converse of Lemma~\ref{lem:weighted-on-all-paths}.
\begin{lemma}\label{lem:atomic-to-weighted-reading-down}
	For every atomic counter automaton $\Aa$ over alphabet $A$ there is a deterministic transducer
	transducer
	\begin{align*}
		f : \trees A \to \countertrees C
	\end{align*}
	that produces only down counter trees, and a formula $\varphi$ of weighted \mso, such that  $\Aa$ accepts a tree $t$ if and only if every full path $\pi$ satisfies
	\begin{align*}
		f(t)\restrict \pi \models \varphi.
	\end{align*}
\end{lemma}
\begin{mproof}
	\begin{center}
		(TODO estimated at one paragraph)
	\end{center}
\end{mproof}








\begin{lemma}\label{lem:tape-down}
	Let 
	\begin{align*}
		f: \trees A \to \countertrees C 
	\end{align*}
	be a deterministic transducer, which  produces only down counter trees. There is a finite set $B$ and deterministic transducers
	\begin{align*}
		g : \trees A \to \countertrees {C \times B}\\
		h : \trees A \to \trees B
	\end{align*}
	such that for every tree $t \in \trees A$ and nodes $x \le xy$, if $b \in B$ is the label of $x$ in $h(t)$, then
	\begin{align*}
		val_{f(t|_x)}(c,y)  = val_{g(t)}((c,b),xy)
	\end{align*}
\end{lemma}
\begin{mproof}
	(TODO tape construction, estimated at 5 paragraphs)
\end{mproof}



We now establish the first part of Lemma~\ref{lem:for-all-at-cost-of-nondeterminism}, not that we do not use nondeterminism here.
\begin{lemma}\label{lem:every-subtree-is-actually-atomic}
If  $\Aa$ is an atomic counter automaton, then
\begin{align*}
			\set{t \otimes X : \mbox{$\Aa$ accepts the subtree $t|_x$ for every $x \in X$}}
\end{align*}
is recognised by an atomic counter automaton.
\end{lemma}
\begin{mproof}
	Apply Lemma~\ref{lem:atomic-to-weighted-reading-down} to $\Aa$, yielding a transducer 
	\begin{align*}
		f : \trees A \to \countertrees C
	\end{align*}
	and a formula $\varphi$ of weighted \wmso+u+u. By the lemma, a subtree $t|_x$ is accepted by $\Aa$ if and only if for every full path $\pi$ in the subtree $t|_x$, 
	\begin{align}\label{eq:weighted-formula-on-a-path}
		val_{f(t|_x)} \restrict \pi \models \varphi.
	\end{align}
	Apply Lemma~\ref{lem:tape-down} to the transducer $f$, yielding transducers $g$ and $h$. For $b \in B$, define $\varphi_b$ to be like $\varphi$, except that instead of reading counter $c$, it reads counter $(c,b)$. By Lemma~\ref{lem:tape-down} we know that if the label of node $x$ in the tree $h(t)$ is $b$, then~\eqref{eq:weighted-formula-on-a-path} is equivalent to
	\begin{align*}
		val_{g(t)} \restrict x\pi \models \varphi_b,
	\end{align*}
	where $x\pi$ is the path obtained by shifting $\pi$ so that its first node becomes $x$. It follows that there is a formula $\psi$ of weighted \wmso+u+u such that for every infinite path $\pi$, not necessarily beginning in the root, we have 
	\begin{align*}
		val_{f(t|_x)} \restrict \pi \models \varphi \qquad \mbox{iff} \qquad h(t) \otimes val_{g(t)} \restrict x\pi \models \psi.
	\end{align*}
	Define $\psi'$ to be the formula which is true in a word 
	\begin{align*}
		w \otimes v \qquad \mbox{with } w\in  (B \times \bar \Nat^{C})^\omega \mbox{ and } v \in  \set{0,1}^\omega
	\end{align*}	
	if $\psi$ is true in every suffix of $w$ that begins with a position that has label $1$ in $v$. This is also a formula of weighted \wmso+u+u. By the properties of $\psi$, it follows that  a tree $t \otimes X$ belongs to the language from the statement of the lemma if and only if $\psi'$ is true in every path of the tree
	\begin{align*}
		h(t) \otimes val_{g(t)} \otimes X.
	\end{align*}
	Therefore, by Lemma~\ref{lem:weighted-on-all-paths}, the language in the statement of the lemma is recognised by an atomic counter automaton.	
\end{mproof}




\subsection{From nondeterministic atomic counter automata to flat \wmsoup automata.}
\label{sec:nondeterministic-to-inf-sup}
In this section, we prove the following lemma, which says  that atomic counter automata are captured by flat \wmsoup automata.  

\begin{lemma}\label{lem:inf-sup-capture-atomic}
For every nondeterministic atomic counter automaton one can compute an  equivalent  flat \wmsoup automaton.
\end{lemma}



\begin{lemma}\label{lem:parity-witness}
	For every $t \in \countertrees C$ and counter $c \in C$, there exists a set of nodes $X$ such that:
	\begin{enumerate}
		\item Counter $c$ is tail unbounded on every path that visits $X$ infinitely often; and
		\item Counter $c$ is bounded in every $X$-factor.
	\end{enumerate}
	Furthermore, if $X$ satisfies both properties above, then counter $c$ is tail unbounded on a path $\pi$ if and only if the path visits $X$ infinitely often.
\end{lemma}
\begin{mproof}
	Intuitively speaking, we define $X$ to be the set of nodes where counter $c$ exceeds its biggest previous value. More formally, we define a sequence of sets $X_0,X_1,\ldots$ by induction as follows. Define $X_0$ to be the root of $t$. For $n > 0$, define the set $X_n$ by induction as follows
\begin{align*}
	X_{n} = \set{xy : x \in X_{n-1} \mbox{ and $y$ is a minimal node with $val_{t|_x}(c,y) \ge n$}}.
\end{align*}
\begin{center}
	(TODO : complete )
\end{center}
\end{mproof}

The properties 1 and 2 in Lemma~\ref{lem:parity-witness} can be seen as sets of trees 
\begin{align*}
	t \otimes X \in \countertrees C \otimes \trees{\set{0,1}}.
\end{align*}
Therefore, it makes sense to ask if these properties are recognised by flat \wmsoup automata.
Suppose that these properties are recognised by flat \wmsoup automata; we will show this later in the section. Then Lemma~\ref{lem:inf-sup-capture-atomic} follows, as we show below.


\begin{mproof}[of Lemma~\ref{lem:inf-sup-capture-atomic}]
	Let $\Aa$ be an atomic \wmsoup counter automaton, with counters  $\set{c_1,\ldots,c_n}$ and a transducer
	\begin{align*}
		f : \trees A \to \countertrees {\set{c_1,\ldots,c_n}}.
	\end{align*}
Given a tree $t$, the automaton guesses sets of nodes  $X_1,\ldots,X_n$ and checks that:
 \begin{itemize}
 	\item[(a)] for every $i \in \set{1,\ldots,n}$, the set $X_i$ satisfies properties 1 and 2 in Lemma~\ref{lem:parity-witness} with respect to counter $c_i$ in the counter tree $f(t)$; and 
	\item[(b)] for every path $\pi$, the accepting set $\Uu$ of $\Aa$ contains the set
	\begin{align*}
		 \set{ c_i  : \mbox{$\pi$ visits $X_i$ infinitely often}}
	\end{align*}
 \end{itemize}
We have assumed that  for  every fixed $i$, the condition (a) can be done by a flat \wmsoup automaton.    Condition (b) is recognised by a parity automaton, and therefore by a flat \wmsoup automaton thanks to Lemma~\ref{lem:flat-simulate-parity}. Therefore, the conjunction of conditions  (a) and (b) is recognised by a flat \wmsoup automaton, thanks   closure under intersection from Lemma~\ref{lem:puzzles-closed-under-intersection}. The guessing of the sets $X_1,\ldots,X_n$ is done using nondeterminism.
\end{mproof}

Therefore, it remains to show that the properties 1 and 2 in Lemma~\ref{lem:parity-witness} are recognised by flat \wmsoup automata. We begin with property 2.


\begin{lemma}\label{lem:tree-inf-sup-capture-bounded-unbounded}
	There is a flat \wmsoup automaton recognising the language
	\begin{align*}
		\set{t \otimes X : \mbox{$c$ is bounded in every $X$-factor}}
	\end{align*}	
\end{lemma}
\begin{mproof}(rough sketch)
	This is a language of the form $\mathsf{AG}K$, as in the assumption of Lemma 19 in~\cite{BojanczykTorunczyk12}. Therefore,  by the conclusion of the lemma, it is recognised by a puzzle, as defined in~\cite{BojanczykTorunczyk12}. The puzzle produced in Lemma 19 has the property, that it only requires counters to be bounded in every $c$-cut-factor. Such puzzles are a special case of flat \wmsoup automata, where for every state $q$, there are no counters in $\biginf q$ and $\smallsup q$ is all counters.
\end{mproof}



\begin{lemma}\label{lem:tree-inf-sup-capture-bounded-unbounded}
	There is a flat \wmsoup automaton recognising the language
	\begin{align*}
		\set{t \otimes X : \mbox{$c$ is tail unbounded on every path that visits $X$ infinitely often}}
	\end{align*}	
\end{lemma}
\begin{mproof}
	\begin{center}
		(todo : estimated at 2 pages)
	\end{center}
\end{mproof}




>>>>>>> External Changes


==> simulation <==
\subsection{Simulation}

Let $t,t'$ be virtual runs. A simulation 
\begin{align*}
	f : t \to t'
\end{align*}
is defined to be a partial from nodes of $t$ to  nodes of $t'$, such that:

\begin{itemize}
	\item  the  descendant relation is preserved;
	\item the function is defined on the root and all ports of $t$;
	\item the root is mapped to the root, ports are mapped to ports.
\end{itemize}
A simulation yields a factorisation of $t$, defined as follows. For each node $x$ in the domain of $t$, there is a factor which contains $x$ and all of its descendants that can be reached by a path not passing through other nodes in the domain of $f$.

Suppose that $\pi$ is a finite path in $t$, which connects two nodes $x$ and $y$ in the domain of $f$. We write $f(\pi)$ for the path in $t'$ which connects  $f(x)$ and $f(y)$. Define the $f$-depth of a node  $x$ in $t$ to be the number of ancestors of $x$ that are in the domain of $f$.  Suppose that $(\epsilon_n)_{n \in \Nat}$ is a sequence of real numbers. A simulation $f$ is called \emph{converging with rate $(\epsilon_n)_{n \in \Nat}$} if for every nodes $x$ and $y$ in the domain of $t$, if $\pi$ is the path from $x$ to $y$, then the distance between the labels of $\pi$ and $f(\pi)$ is  at most $\epsilon_n$, where $n$ is the $f$-depth of $n$. The convergence rate of a simulation is the smallest rate for which it converges.


\begin{lemma}\label{lem:simulation-transfers-bad-comb}
	Suppose that $f: t' \to t$ is a simulation of a virtual run in a run, which has a convergence rate that converges to zero. If $t'$ has a bad comb, then $t$ violates the boundedness acceptance condition.
\end{lemma}
\begin{mproof}
	Let $(\epsilon_n)_{n \in \Nat}$ be the rate of the simulation, which is assumed to converge to zero. 
	Suppose that   $t'$ contains a bad $c$-comb for some counter $c$, and them infinite path in this comb is a sequence of edges $e_1 e_2 \ldots$. Let $f(e_1),f(e_2),\ldots$ be the infinite path in $t$ which is the image of the bad comb under $f$.  
	\begin{center}
		...fill in...should be easy...
	\end{center}
\end{mproof}


\begin{lemma}\label{lem:sufficient-condition-for-closeness}
	Let $t$ be a  term, and let $\epsilon > 0$. There is a finite set of ports in $X$ such that the following condition is sufficient for a term $t'$ to be  $\epsilon$-close to $t'$: 
	\begin{quote}
		(*) There is a simulation $f : t' \to t$ which has a convergence rate bounded by  $\epsilon$, and such that the image of $f$ contains $X$.
	\end{quote}
	\end{lemma}

==> trash.tex <==
\subsection{Configuration structures}
The idea behind the decidability results is that to every database-driven system over a class of structures $\Cc$,  we will assign a structure, called its configuration structure, such that a) the configuration structure will be definable over the \fraisse limit of $\Cc$; and b) the emptiness problem for the system will be definable by an appropriate logical formula evaluated in the configuration structure.








\begin{remark}
	At the end of the above proof,  it is tempting to consider a simpler graph, where vertices $\bar x$-types and  there is an edge from $\tau$ to $\tau'$ there are $\psi$-connected $n$-tuples $\bar b$  and $\bar b'$ such that
		\begin{enumerate}
			\item  $\tau$ is type  of 	the valuation which maps $\bar x$ to $\bar b$;
					\item  $\tau'$ is type  of 	the valuation which maps $\bar x$ to $\bar b'$;
		\end{enumerate}
One might think that  $\thesemantics{TC_{\bar x \bar y} \psi}$ would be equal to the set of $\bar x \bar y$-types $\tau$ such that  the above graph contains a path from the type of the $\bar x$ variables in $\tau$ to the type of the $\bar y$ variables in $\tau$ (seen as a $\bar y$-type). The right-to-left inclusion would fail in such a reasoning.  	
	Consider for instance the case when $\str A$ is the rational numbers with their ordering, and $\psi(x,y)$ holds if $x<y$. Then $\phi(x,y)$ also holds if and only if $x<y$
		(since $<$ is transitive). However, if $x,y$ are any two rational numbers then there is a path from the type of $x$ to the type of $y$ in the simpler graph (since all rational numbers have the same type, and there is a path in the case when $x<y$), but if $y<x$ then the type of $(x,y)$ is not in $\thesemantics \phi$.\end{remark}
	
\subsection{Evaluation for definable  structures}	

\paragraph*{Complexity of evaluation}
The \emph{evaluation problem} for fixpoint logic is the following decision problem.
\begin{quote}
{\upshape \begin{tabular}{ll}
  \textbf{Parameters:} & A structure $\str A$ and a sentence $\phi$ of least fixpoint logic,\\
  \textbf{Input:}	& a structure $\str B$ definable  over $\str A$\\
  \textbf{Decide:}	& does $\phi$ hold in $\str B$?
  \end{tabular}
 } 
 \end{quote}



\begin{lemma}\label{lem:transfer}
	If $I$ is an interpretation, then for sentence formula $\varphi$ of least fixpoint logic, one can compute a sentence $I(\varphi)$ of least fixpoint logic such that 
	\begin{align*}
		I(\str A) \models \varphi \qquad \mbox{iff}\qquad \str A \models I(\varphi).
	\end{align*}
	holds whenever $I(\str A)$ is defined. The number of variables in $I(\varphi)$ is the number of variables in $\varphi$ times the dimension of $I$. 
\end{lemma}



	
	However, for $\tau\in\typesreg{\bar x\bar y}$ it is not necessarily true that $\tau\in\thesemantics\phi$ if there is a directed path in $H_\psi$ from the projection
	of $\tau$ to $\typesreg{\bar x}$ to the projection of $\tau$ to $\typesreg{\bar y}$.	
Consider for instance the case when $\str A=\str B$ are the rational numbers with their ordering, and $\psi(x,y)$ holds if $x<y$. Then $\phi(x,y)$ also holds if and only if $x<y$
	(since $<$ is transitive). However, if $x,y$ are any two rational numbers then there is a path from the type of $x$ to the type of $y$ in $H_\psi$ (since all rational numbers have the same type, and there is a path in the case when $x<y$), but if $y<x$ then the type of $(x,y)$ is not in $\thesemantics \phi$.

\begin{proof}[of Lemma~\ref{lem:reachability}]			
	Suppose that $\tau\in\thesemantics\phi$.
	Let $\bar u\bar v$ be any valuation which has type~$\tau$.	
	Then there exists a $\psi$-path $\bar u_0,\bar u_1\ldots,\bar u_r$
	from $\bar u$ to $\bar v$.
For $i=0,1,\ldots$ let $\tau_i$ denote the type of the valuation $\bar u\bar u_i$.
By definition of the graph $G_\psi$, the types $\tau_0,\ldots,\tau_r$ 
form a directed path in $G_\psi$. This proves one implication of the lemma.
	 
	 Conversely, 	 
	 for any path $\tau_0,\ldots,\tau_r$ in the graph $G_\psi$
	 we inductively construct a corresponding $\psi$-path $\bar u_0,\ldots,\bar u_r$ of valuations  such that for $k=0,1,\ldots,r$ the type of the valuation $\bar u_0\bar u_k$ is $\tau_k$.
	 The initial type $\tau_0$ is by assumption a type of a tuple of the form 
	 $\bar u_0\bar u_0$, and the $\psi$-corresponding path contains only the valuation $\bar u_0$. In the inductive step, suppose that a $\psi$-path $\bar u_0,\bar u_1,\ldots,\bar u_{k}$ 
	 of valuations has been already constructed and that the type of the valuation $\bar u_0\bar u_k$ is $\tau_k$.	 Since there is an edge from $\tau_{k}$ to $\tau_{k+1}$ in $G_\psi$, it follows that there is a triple of valuations $\bar u,\bar v_1,\bar v_2$ such that:
 	\begin{enumerate}
 		\item 	 $\bar v_1$ and $\bar v_2$ are $\psi$-connected,
 		\item 	the type of the valuation $\bar u\bar {v_1}$      for $\bar x\bar y$ is $\tau_k$,
 		\item 	the type of the valuation  $\bar u\bar {v_2}$     for $\bar x\bar y$ is $\tau_{k+1}$.
 	\end{enumerate}
	 Since $\str A$ is homogeneous and the tuple $\bar u \bar v_1$ has the same type as the tuple $\bar u_0\bar u_{k}$,
	 there is an automorphism of $\str A$ such that the induced 
 automorphism of $\str B$ maps the first tuple to the second one (c.f. proof of Lemma~\ref{lem:orbit}).
 Let $\bar u_{k+1}$ be the image of the tuple $\bar v_2$ under the induced automorphism.
Then  $\bar u_{k}$ and $\bar u_{k+1}$ are $\psi$-connected and  $\bar u_0\bar u_{k+1}$ has type $\tau_{k+1}$.
This ends the inductive step in the construction of the $\psi$-path from $\bar u_0$ to $\bar u_r$. 
Hence, there is a $\psi$-path from $\bar u_0$ to $\bar u_r$, so $\bar u_0\bar u_r$ satisfies $\phi$, proving that $\tau_r\in\thesemantics \phi$.
\end{proof}


\subsection{old}
The rest of Section~\ref{sec:evaluating-fixpoints} is devoted to showing Theorem~\ref{thm:evaluate-fixpoint-logics}. 
\medskip

Fix the homogeneous structure $\str A$ as in the theorem. We call the elements of $\str A$ \emph{atoms}.
Define the \emph{type} of a tuple of atoms to be the isomorphism type of the
structure generated by these atoms, with special constants for all atoms of
the tuple. The type of an $n$-tuple of atoms can be represented in space
$\poly(f(n))$, and the same space is sufficient to decide if a given structure is  the type of some tuple of atoms; here we use the assumption that embeddability is decidable in \pspace.

Now fix a definable structure $\str B$.  We call the components of the domain
of $\str B$ \emph{colors}.  The elements of $\str B$ will be referred to as,
simply, \emph{elements}.  Each element is described by its color together with
a tuple of atoms of appropriate length making true the quantifier-free formula
defining its color.  Define the \emph{type} of a tuple of elements to be the
colors of each element together with the type of the tuple of atoms
formed by all the atoms associated to each element.  If $\bar x$ is a tuple
of $l$ variables, then define $\typesreg {\bar x}$ to be the set of possible types
of valuations of $\bar x$. The number of elements in $\typesreg {\bar x}$ is as
in~\eqref{eq:lfp-time} and the the space required to represent an element of
$\typesreg {\bar x}$ is as in~\eqref{eq:lfp-space}.

\begin{lemma}\label{lem:orbit}
  Consider a formula of least fixpoint logic over the schema of $\str B$. If two
  valuations of the free variables have the same type, then both satisfy the
  formula or both do not satisfy it.
\end{lemma}
	\begin{proof}
          Assume that $\bar x$ and~$\bar y$ are two tuples of \emph{elements}
          (of $\str B$) of the same type. Let $\bar u,\bar v$ obtained from
          concatenating the atoms associated to the elements in $\bar x$ and
          $\bar y$, respectively. By definition $\bar u$ and $\bar v$ have the
          same type. Hence there is a partial isomorphism of $\str A$ mapping
          $\bar u$ to $\bar v$. By homogeneity of $\str A$ this partial
          isomorphism extends to an automorphism $\alpha$ of $\str A$.

          This automorphism $\alpha$ induces an automorphism on $\str B$ which
          transforms each element by applying $\alpha$ to its associated atoms while leaving
          the color unchanged.  This mapping of $\str B$ is an automorphism,
          since the relations of $\str B$ are defined by formulas without
          constants, so they are preserved by $\alpha$.


          Since our formula do not use constants, they are invariant under the
          automorphisms of~$\str B$. It follows that any formula that is
          satisfied by $\bar x$ is also satisfied by $\bar y$.
	\end{proof}
	


By the above lemma, we can associate to each formula $\phi$ with free variables
$\bar x$ a subset of $\typesreg {\bar x}$, denoted by $\thesemantics \phi$,
corresponding to the types of tuples of elements making $\phi$ true. Then if
$\phi$ is a sentence, $\thesemantics\phi$ is empty iff $\phi$ does not hold in
$\str B$. Therefore the following proposition implies Theorem~\ref{thm:evaluate-fixpoint-logics}.

	
\begin{proposition}\label{prop:thesemantics}
		The set $\thesemantics\phi$ can be computed in time and space as described in Theorem~\ref{thm:evaluate-fixpoint-logics}.		
\end{proposition}

We prove Proposition~\ref{prop:thesemantics} by induction on the structure of the formula $\phi$.
It is essentially the classical fixpoint evaluation algorithm except that the
computation is done at the level of types instead of the elements of the
domain. Correctness is guaranteed by homogeneity and Lemma~\ref{lem:orbit}.

\paragraph*{Base case}
The base case is when $\phi$ is of the form $R(\bar x)$ for some relational
symbol $R$ of~$\str B$.  Then $\thesemantics \phi$ is computed by selecting
those of $\typesreg {\bar x}$ which satisfy the formula defining the relation
$R$ in~$\str B$. This amounts to evaluating the quantifier-free formula
defining $R$ (of size at most $\size(\str B)$) in $m$ structures, where $m$ is
the cardinality of $\typesreg{\bar x}$ and each of those structures is
represented in space~\eqref{eq:lfp-space}.  This gives the required time and
space for computing $\thesemantics \phi$.
 % $\poly(\size(\str B))\cdot m$  which is as required in~\eqref{eq:lfp-time}, and space as required in~\eqref{eq:lfp-space}.

\paragraph*{First order constructs}
The case when $\phi$ is a boolean combination of formulas $\phi_1,\ldots,\phi_k$ with free variables $\bar x$
is easy, since then $\thesemantics\phi$ is the corresponding boolean combination of subsets $\thesemantics{\phi_1},\ldots,\thesemantics{\phi_k}$ of $\typesreg{\bar x}$.
Now, consider the case when $\phi$ is of the form $\exists \bar y.\psi$, where $\psi$ has free variables~$\bar x\bar y$.
Then $\thesemantics\phi$ is the image of $\thesemantics \psi$
under the projection from $\typesreg{\bar x \bar y}$ to $\typesreg{\bar x}$.
The image of a given element $\tau\in\typesreg{\bar x\bar y}$ under this projection
can be computed in time $\poly(f(l)\cdot \dim (\str B))$. This gives the required time and space for computing $\thesemantics \phi$.  

% This handles all constructs of first order logic.




\paragraph*{Fixpoint operation}
Consider the case of a formula $\phi$ of the following form
\begin{align}
	\label{eq:lfp3}
	\text{let }R(\bar x)=\lfp\ \psi\text { in }R(\bar z)
\end{align}
(see Remark~\ref{rem:lfp1} for why this special case is sufficient).
We may first reduce this form to the special case when the formula $\psi$ 
has no parameters. Indeed, if $\bar y$ are the parameters of $\psi$ in~\eqref{eq:lfp3}, then
	the formula~\eqref{eq:lfp3}
	is equivalent to the formula
	\begin{align*}%\label{eq:lfp2}\tag{lfp''}
		\text{let }S(\bar x,\bar y)=\lfp\ \hat\psi\text { in }S(\bar z,\bar y),
	\end{align*}
	where $\hat\psi$ is obtained from $\psi$ by replacing each occurrence of 
	a predicate $R(\bar u)$ by $S(\bar u, \bar y)$.


Therefore, we may assume that $\phi$ is a formula as in~\eqref{eq:lfp3},
such that $\bar x$ are all the free variables of the formula $\psi$.
 Let $n$ be the arity of the symbol $R$, which coincides with the length of the tuples $\bar x$ and $\bar z$.


We define a sequence $\psi_0,\psi_1,\ldots$ of formulas with free variables $\bar x$ as follows.
	Let $\psi_0=\bot$. 
	For $k=0,1,2,\ldots$, let $\psi_{k+1}$ be the formula $\psi$ in which each predicate $R(\bar u)$
	is replaced by $\psi_k(\bar u)$.
	
\begin{lemma}
We have
	\begin{align}\label{eq:psiseq}
	\thesemantics{\psi_0}\subset\thesemantics{\psi_1}\subset\thesemantics{\psi_2}\subset\ldots
	\end{align}
	and the sequence stabilizes after at most $t$ steps, where $t$ is as in~\eqref{eq:lfp-time}.
	Moreover, $\thesemantics {\phi}$ is equal to the ultimate value of the sequence.
\end{lemma} 
\begin{proof} 
Let $\Rr\mapsto\Rr'$ be the mapping of $n$-ary relations described in Section~\ref{sec:fixpoint}, which maps a relation $\Rr$ to the relation $\Rr'$ consisting of those tuples which satisfy the formula $\psi(\bar x)$ in the structure~$\str B$ extended by the relation $\Rr$. Recall that this mapping is monotone, and $\phi$ holds in $\str B$ iff $R(\bar z)$ holds in the extension of $\str B$ by the least fixpoint of the mapping $\Rr\mapsto\Rr'$.
 
 Define a sequence $\Rr_0,\Rr_1,\ldots$ of $n$-ary relations
where
 $\Rr_0$ is the empty relation
and $\Rr_{k+1}=\Rr_{k}'$ for $k=0,1,2,\ldots$
It follows from monotonicity of the mapping $\Rr\mapsto\Rr'$ that these relations form an increasing sequence:
\begin{align}\label{eq:rseq}
\Rr_{0}\subset\Rr_{1}\subset\Rr_{2}\subset\ldots
\end{align}


For a type $\tau\in \thesemantics{\psi_k}$, let $\langle\tau\rangle$ denote the set of $n$-tuples of elements of $\str B$ which, treated 
as a valuation for the variables $\bar x$, have type $\tau$.
By an easy induction on $k$ we get:
	$$\Rr_k=\bigcup\set{\langle\tau\rangle:\ \tau\in\thesemantics{\psi_k}}\qquad\text{for }k=0,1,2,\ldots.$$

In particular, from~\eqref{eq:rseq} the inclusions in~\eqref{eq:psiseq} follow.
Since $\thesemantics {\psi_k}\subset \typesreg {\bar x}$  for all $k$,
 the sequence~\eqref{eq:psiseq} must stabilize after at most $t$ steps, where $t$ is as in~\eqref{eq:lfp-time}.
It follows that $\Rr_t=\Rr_{t+1}$, so $\Rr_t$ is the least fixpoint of the mapping $\Rr\mapsto\Rr'$.
Therefore, $\thesemantics \phi=\thesemantics {\psi_t}$, proving the lemma.
\end{proof}


As a consequence, in order to compute $\thesemantics \phi$ it suffices to compute $\thesemantics {\psi_k}$ for $k=0,1,2,\ldots$ until stabilization is reached after at most $t$ steps, where $t$ is as in~\eqref{eq:lfp-time}.
Overall, this gives the required time bound.

\paragraph*{Transitive closure operation}
Now consider the case when $\phi$ is defined using the transitive closure operator from a simpler formula $\psi$. 
 Again, we may first reduce to the case when $\psi$ has no parameters.
Indeed, the transitive closure $R^\ast(\bar x,\bar x',\bar y)$ of the relation $R(\bar x,\bar x',\bar y)$
with  $k$ parameters $\bar y$
can be computed in two steps:
\begin{itemize}
	\item first compute the transitive closure $S^\ast(\bar x,\bar y,\bar x',\bar y')$ of 
the relation $S$, where $S(\bar x,\bar y,\bar x',\bar y')$ holds if and only if
$(\bar y=\bar y')$ and $R(\bar x,\bar x',\bar y)$;
	\item then $R^\ast(\bar x,\bar x',\bar y)$ is equivalent to $S^\ast(\bar x,\bar y,\bar x',\bar y)$.
\end{itemize}




So let us assume that $\phi$ is defined  by the transitive closure operation from a formula $\psi$, where $\psi$ has $2n$ free variables $\bar x\bar y$, and is considered as a binary relation on $n$-tuples.

	Let $\bar u$ and $\bar v$ be two valuations for $\bar x$.
	We say that  $\bar u$ and $\bar v$ are $\psi$-\emph{connected}
	if  $\bar u\bar v$, treated as a valuation for $\bar x\bar y$,
	satisfies the formula $\psi$ (this is usually not a symmetric relation).
	A \emph{$\psi$-path} is a finite sequence of valuations for $\bar x$, where each two consecutive valuations are $\psi$-connected.
	It follows from the definition of the transitive closure operation that
	a valuation $\bar u\bar v$ satisfies the formula $\phi$ if and only if 
	there is a $\psi$-path from $\bar u$ to $\bar v$.

Consider the directed graph $G_\psi$ where:
\begin{itemize}
	\item The nodes are the elements of $\typesreg{\bar x\bar y}$,
	\item 
There is an edge from $\tau_1$ to $\tau_2$
	if there is a triple of valuations $\bar u,\bar {v}_{1},\bar {v}_{2}$
	of the variables $\bar x$ such that 
	\begin{enumerate}
		\item 	 $\bar v_1$ and $\bar v_2$ are $\psi$-connected,
		\item 	the type of the valuation $\bar u\bar {v_1}$      for $\bar x\bar y$ is $\tau_1$,
		\item 	the type of the valuation  $\bar u\bar {v_2}$     for $\bar x\bar y$ is $\tau_2$.
	\end{enumerate}
\end{itemize}
% A \emph{diagonal} node is a node in $G_\psi$ which is the type of a tuple $\bar u\bar {v}$ with $\bar u=\bar {v}$.

Let $\tau\in\typesreg{\bar x\bar y}$ and let $\bar u\bar v$ be a  valuation for the variables $\bar x\bar y$ of type $\tau$.
By $\tau_0$ we denote the type of the tuple $\bar u\bar u$;
the type $\tau_0$ does not depend on the choice of $\bar u\bar v$.

\begin{lemma}\label{lem:reachability}
	Let $\tau\in\typesreg{\bar x\bar y}$. Then $\tau\in \thesemantics \phi$
	if and only if there is a directed path in $G_\psi$ from the node $\tau_0$
 to $\tau$.
\end{lemma}

Therefore, computing $\thesemantics \phi$ amounts to computing directed reachability in the graph $G_\psi$. This can be computed nondeterministically in space  depending logarithmically on the size of the graph, and the size is as in~\eqref{eq:lfp-time}. By Savitch's theorem, this can be also done deterministically in space as in~\eqref{eq:lfp-space}.

\begin{remark}
	It is tempting to consider a simpler graph $H_\psi$ instead of $G_\psi$, where
	\begin{itemize}
		\item The nodes are the elements of $\typesreg{\bar x}$,
		\item 	There is an edge from $\tau_1$ to $\tau_2$
		if there is a pair of valuations $\bar {v}_{1},\bar {v}_{2}$
		of the variables $\bar x$ such that 
			 	 $\bar v_1$ and $\bar v_2$ are $\psi$-connected.			
	\end{itemize}
	% A \emph{diagonal} node is a
	
	However, for $\tau\in\typesreg{\bar x\bar y}$ it is not necessarily true that $\tau\in\thesemantics\phi$ if there is a directed path in $H_\psi$ from the projection
	of $\tau$ to $\typesreg{\bar x}$ to the projection of $\tau$ to $\typesreg{\bar y}$.	
Consider for instance the case when $\str A=\str B$ are the rational numbers with their ordering, and $\psi(x,y)$ holds if $x<y$. Then $\phi(x,y)$ also holds if and only if $x<y$
	(since $<$ is transitive). However, if $x,y$ are any two rational numbers then there is a path from the type of $x$ to the type of $y$ in $H_\psi$ (since all rational numbers have the same type, and there is a path in the case when $x<y$), but if $y<x$ then the type of $(x,y)$ is not in $\thesemantics \phi$.
\end{remark}
\begin{proof}[of Lemma~\ref{lem:reachability}]			
	Suppose that $\tau\in\thesemantics\phi$.
	Let $\bar u\bar v$ be any valuation which has type~$\tau$.	
	Then there exists a $\psi$-path $\bar u_0,\bar u_1\ldots,\bar u_r$
	from $\bar u$ to $\bar v$.
For $i=0,1,\ldots$ let $\tau_i$ denote the type of the valuation $\bar u\bar u_i$.
By definition of the graph $G_\psi$, the types $\tau_0,\ldots,\tau_r$ 
form a directed path in $G_\psi$. This proves one implication of the lemma.
	 
	 Conversely, 	 
	 for any path $\tau_0,\ldots,\tau_r$ in the graph $G_\psi$
	 we inductively construct a corresponding $\psi$-path $\bar u_0,\ldots,\bar u_r$ of valuations  such that for $k=0,1,\ldots,r$ the type of the valuation $\bar u_0\bar u_k$ is $\tau_k$.
	 The initial type $\tau_0$ is by assumption a type of a tuple of the form 
	 $\bar u_0\bar u_0$, and the $\psi$-corresponding path contains only the valuation $\bar u_0$. In the inductive step, suppose that a $\psi$-path $\bar u_0,\bar u_1,\ldots,\bar u_{k}$ 
	 of valuations has been already constructed and that the type of the valuation $\bar u_0\bar u_k$ is $\tau_k$.	 Since there is an edge from $\tau_{k}$ to $\tau_{k+1}$ in $G_\psi$, it follows that there is a triple of valuations $\bar u,\bar v_1,\bar v_2$ such that:
 	\begin{enumerate}
 		\item 	 $\bar v_1$ and $\bar v_2$ are $\psi$-connected,
 		\item 	the type of the valuation $\bar u\bar {v_1}$      for $\bar x\bar y$ is $\tau_k$,
 		\item 	the type of the valuation  $\bar u\bar {v_2}$     for $\bar x\bar y$ is $\tau_{k+1}$.
 	\end{enumerate}
	 Since $\str A$ is homogeneous and the tuple $\bar u \bar v_1$ has the same type as the tuple $\bar u_0\bar u_{k}$,
	 there is an automorphism of $\str A$ such that the induced 
 automorphism of $\str B$ maps the first tuple to the second one (c.f. proof of Lemma~\ref{lem:orbit}).
 Let $\bar u_{k+1}$ be the image of the tuple $\bar v_2$ under the induced automorphism.
Then  $\bar u_{k}$ and $\bar u_{k+1}$ are $\psi$-connected and  $\bar u_0\bar u_{k+1}$ has type $\tau_{k+1}$.
This ends the inductive step in the construction of the $\psi$-path from $\bar u_0$ to $\bar u_r$. 
Hence, there is a $\psi$-path from $\bar u_0$ to $\bar u_r$, so $\bar u_0\bar u_r$ satisfies $\phi$, proving that $\tau_r\in\thesemantics \phi$.
\end{proof}


